Gumbel Distillation for Parallel Text Generation

The slow, sequential nature of autoregressive (AR) language models has driven the adoption of parallel decoding methods. However, these non-AR models often sacrifice generation quality as they struggle to model the complex joint distribution of token sequences. To narrow this performance gap, we introduce Gumbel Distillation, a novel distillation technique that enables parallel decoders to learn this distribution effectively. Our method leverages the Gumbel-Max trick to create a deterministic mapping from a latent Gumbel noise space to the output tokens of a high-performing AR teacher. As a model-agnostic technique, Gumbel Distillation seamlessly integrates with diverse parallel decoding architectures, including MDLM and BD3-LM. Experiments on LM1B and OpenWebText show that Gumbel Distillation substantially improves the generation quality of parallel language models, achieving a 30.0% improvement in MAUVE score and 10.5% in generative perplexity over MDLM trained on OpenWebText dataset. Code available at https://github.com/hxixixh/gumbel-distill.

==> floats/algo_gumbel.tex <==
% \begin{algorithm}[t!]
% \caption{Gumbel Distillation}
% \label{alg:gumbel_distill}
% \begin{algorithmic}[1]
% \State \textbf{Input:} Autoregressive teacher model $p^*$, parallel student model $p_\theta$.

% \vspace{0.5em}
% \Statex \textcolor{gray}{\textit{// Step 1: Obtain Gumbel-token pairs from teacher as distillation data}}
% \State Construct dataset $\mathcal{D} = \{(\xi^{(i)}_{1:n}, x^{(i)}_{1:n})\}_{i=1}^N$ by obtaining pairs such that:
% \begin{itemize}
%     \item $x_{1:n}$ is the ground truth token sequence.
%     \item $\xi_{1:n}$ corresponds to $x_{1:n}$ as sampled from $p^*(\cdot|\xi_{1:n})$ via the Gumbel-Max trick.
%     \item This dataset can be obtained either by sequential sampling from $p^*$ or by efficient posterior recovery (introduced in Theorem 3.1) from an existing corpus.
% \end{itemize}

% \vspace{0.5em}
% \Statex \textcolor{gray}{\textit{// Step 2: Train the parallel student model on the distilled dataset}}
% \State Train the parallel student $p_\theta$ by minimizing the negative log-likelihood:
% $$ \min_\theta \mathcal{L}(\theta) = \mathbb{E}_{(\xi, x) \sim \mathcal{D}} [-\log p_\theta(x|\xi)] $$

% \State \textbf{Output:} Trained parallel student model $p_\theta$.
% \end{algorithmic}
% \end{algorithm}



==> sections/backup.tex <==
Old abstract:

% Predicting multiple tokens have emerged as a powerful paradigm for generative modeling, including discrete diffusion model and multi-token prediction, yet they often lag behind autoregressive models in performance or require numerous sampling steps\xixi{remove this if gumbel does not perform well for low nfe}, limiting their practical utility. In this work, we introduce a novel and efficient technique to accelerate both training and inference for multi-token prediction or discrete diffusion models. Our method leverages the Gumbel-Max trick within a Rectified Flow framework, establishing a straight and efficient transport path from Gumbel noise to data tokens. This approach facilitates a highly effective distillation of powerful pretrained autoregressive models into a non-autoregressive, few-step diffusion student. We demonstrate the efficacy and simplicity of our method by integrating it with existing state-of-the-art discrete diffusion frameworks, including MDLM and Block Diffusion, we also integrate it with multi-token predcition framework. Experimental results validate that our proposed Gumbel-Rectified Flow significantly enhances inference speed while maintaining high-quality generation, thereby bridging the gap between the generative capabilities of autoregressive models and the efficiency of parallel diffusion.


Old intro:

% The rapid advancement of large language models (LLMs) has been largely driven by the scaling of autoregressive (AR) architectures, which generate text sequentially by predicting one token at a time. While this paradigm excels at capturing the sequential dependencies of language, its token-by-token generation process is inherently slow and inflexible. In response, recent research has turned to explore non-autoregressive alternatives like Masked Diffusion Models (MDMs) \citep{sahoo2024simple, arriola2025block, nie2025large} or Multi-Token-Prediction (MTP) \citep{cai2024medusa, gloeckle2024mtp, liu2024deepseek} strategies, both of which offer significant gains in inference speed and flexibility by generating entire sequences or blocks of text in parallel.

% While promising, this parallelism comes at a cost: these approaches often face a trade-off between speed and quality, and show inferior performance to their autoregressive counterparts. Behind is a fundamental limitation in the conditional independence assumption \citep{song2025ideas} they make during generation:  the models often predict the probability distribution of multiple tokens in parallel, conditioned only on the shared context. This prevents them from modeling the true joint probability of the tokens. While various inference-time algorithms have been designed to mitigate these errors, the underlying architectural limitation remains.

% This motivates the central question of our work: \textit{is it possible to achieve the inference speed of parallel decoding without sacrificing the generative power of autoregressive models?} Our work explores this question within the framework of knowledge distillation, focusing on transferring the capabilities of a powerful, pre-trained autoregressive teacher model to an efficient, non-autoregressive student, such as a multi-token prediction model or a diffusion language model. Furthermore, we hypothesize that the key to successful distillation lies in defining a simple, straight trajectory from noise to data, which drastically simplifies the student's learning task.

% In this work, we introduce \ours{}, a novel and efficient technique designed to accelerate both training and inference for multi-token prediction and discrete diffusion models. Our core idea is to establish a deterministic relation from a simple Gumbel noise distribution to the complex AR teacher distribution for the non-AR student to learn from. While our method operates in a discrete space, we theoretically connect it to the Reflow technique from Rectified Flow, which was developed for continuous domains. We achieve this by leveraging the Gumbel-Max trick to source Gumbel-noise and data-token pairs from a powerful, pre-trained autoregressive model. These pairs are then used to define a conditoinal mapping for the distillation task, which allows a non-AR student model to learn efficiently. This approach enables the student to generate higher-quality outputs in fewer sampling steps, thus closing the performance gap with its AR teacher.

% Our main contributions are as follows:

% \begin{itemize}
%     \item We propose \ours{}, a novel framework that efficiently transfers knowledge from a pre-trained AR model to a non-AR archiecture by creating a deterministic mapping from Gumbel noise to AR-constrained data distribution for the student to learn from.
%     \item We demonstrate the simplicity and effectiveness of our approach by integrating it with state-of-the-art discrete diffusion frameworks including MDLM and BD3-LM. 
%     \item Our extensive experiments validate that our method significantly enhances inference speed while maintaining high-quality generation, successfully bridging the gap between autoregressive performance and parallel decoding efficiency.
% \end{itemize}




























% \subsection{The Gumbel-Max Trick and Posterior Sampling}

% The Gumbel-Softmax trick \citep{jang2017categorical} provides a method to draw samples from a categorical distribution by leveraging the Gumbel distribution. It establishes that sampling from a categorical distribution with logits $l$ is equivalent to finding the index of the maximum value after adding Gumbel-distributed noise to the logits. Formally, for a random vector $g$ whose components are drawn independently from a $\text{Gumbel}(0,1)$ distribution, the following equivalence holds:
% \begin{equation}
%     \text{argmax}(l+g) \sim \text{Categorical}(\text{Softmax}(l))
% \end{equation}
% \qq{make it clear that $l = [l_{i}]$ and $g = [g_i]$ are vectors ...}
% This principle can be used in reverse to define a stochastic mapping from a known data sample to a latent variable. Given a teacher model $f$ that produces logits $l_i = f(x_{<i+1})$ \qq{need to set up in the beginining what a AR model $f$ is, introduce the notations of $x$ and $\ell$, etc.} and a known outcome token $x_{i+1}$ from a sequence, one can derive a corresponding noise vector $g_i$ that is consistent with this outcome. Such a vector $g_i$ must satisfy the argmax constraint:
% \begin{equation}
%     l_i[x_{i+1}] + g_i[x_{i+1}] \ge l_i[k] + g_i[k], \quad \forall k \neq x_{i+1}
%     \label{eq:gumbel_constraint_background}
% \end{equation}
% \qq{need to define notation $ g_i[k]$, what $i$ and $k$ mean, respectively.}
% This allows for the construction of a guidance signal $g$ that is intrinsically linked to the generation of a specific sequence $x$ by a teacher model $f$. It is also possible to do it in a way that if the teacher model's logits $l$ accurately reflect the true data probabilities, the marginal distribution of the resulting signal $g$ remains standard Gumbel, as shown in the Appendix. 

% The posterior sampling approach offers a significant computational advantage. A naive forward process to obtain a consistent $(g, x)$ pair would require sequential, autoregressive generation: sampling $g_i$ and $x_{i+1}$ at each step before computing the next logits $l_{i+1}$. In contrast, the inverse method is highly parallelizable. Since the entire target sequence $x$ is known beforehand, the teacher model $f$ can compute the logits $l_i$ for all positions simultaneously in a single, non-autoregressive forward pass. Subsequently, the posterior sampling of each $g_i$ from its corresponding $l_i$ and $x_{i+1}$ can also be performed in parallel across the sequence length. This allows us to obtain the entire guidance signal $g$ in one pass, avoiding costly sequential computation.








\subsection{The Challenge of Parallel Language Generation} 

\cz{Discuss AR models and parallel models here (multi-token-prediction, masked diffusion, etc; then introduce the problem statement)}

Parallel techniques used in language modeling, such as multi-token prediction and masked diffusion models, are a promising alternative to traditional autoregressive (AR) methods, offering significant gains in inference speed and flexible control over the number of generation steps. However, a fundamental limitation of these methods is the conditional independence assumption during the simultaneous prediction of multiple tokens. 

Consider a simple case of trying to predict the next two tokens after the sentence: “The cat saw the mouse and decided to ...”. For the immediate next two words to be a valid combination, such as “sit down” or “stand up”, there must exist a strong correlation between them. A standard multi-token prediction model would produce the corresponding softmax weights for each position, sample the tokens independently, and generate unwanted combinations such as “sit up” or “stand down”. The same goes for masked diffusion models if we wish to unmask both positions at once. By modeling the joint distribution of a token block as a product of independent marginals, the parallel models fail to capture the local sequential dependencies that AR models inherently model via the chain rule.

To this end, we propose a novel approach that transfers the inherent sequential knowledge from an AR teacher into a parallel student, overcoming the model's architectural limitation at training time.






















% First we introduce a simple distillation process inspired by the re-flow technique in \cite{liu2023flow}. We construct deterministic mappings from a simple noise distribution to the complex distribution of coherent texts by using the AR teacher to create a dataset of $(G,X)$ pairs, where a sequence of Gumbel noise vectors $G$ serves as a latent variable that deterministically generates a corresponding text sequence $X$. The student can then be trained on the texts while being conditioned on the Gumbel signal, thus learning the underlying joint distribution of the tokens. Here, the deterministic relation between $G$ and $X$ is rooted in the Gumbel-Max trick for sampling from categorical distributions.



% \subsubsection{The Gumbel-Max Trick and Posterior Sampling} \label{sec: method_gumbel}
% For a given sequence of tokens $X = (x_1, x_2, \dots, x_L)$, an AR teacher $f_\theta$ models the probability of the next token $x_{i+1}$ conditioned on the preceding context $x_{\leq i}=(x_1, x_2, \cdots, x_i)$ as:
% \begin{equation}
%     p_\theta(x_{i+1} | x_{\leq i}) = \text{Softmax}(l_i), \text{where} ~ l_{i} = f_\theta(x_{\leq i})
% \end{equation}
% Here $l_i \in \mathbb{R}^V$ is a vector of logits over a vocabulary of size $V$ for the token at position $i+1$. 

% The Gumbel-Max trick \citep{gumbel1954statistical, 10.5555/2969033.2969171} provides the mechanism for sampling from the above categorical distribution. Let $g_i \in \mathbb{R}^V$ be a random vector where each component $g_{i,k}$ is drawn independently from $\text{Gumbel}(0,1)$. Then the following property holds:
% \begin{equation}
%     \arg \max_{k \in [V] } (l_{i,k} + g_{i,k}) \sim \text{Categorical}(\text{Softmax}(l_i))
% \end{equation}
% This means that the next token $x_{i+1}$ can be sampled by finding the index of the maximum value in the perturbed logits. By applying the principle autoregressively, we can obtain an entire sequence of Gumbel noise vectors $G = (g_1, g_2, \dots, g_L)$ that deterministically generates a text sequence $X$.

% In practice, we can leverage the Gumbel-Max trick to generate pairs of $(G, X)$ from the teacher model $f_\theta$ in one of two ways: a sequential forward process, as introduced above where we directly simulate the AR generation path, and a more efficient posterior process that can be parallelized.
